Multi-faceted Graph Attention Network for Radar Target Recognition in Heterogeneous Radar Network

Radar target recognition (RTR), as a key technology of intelligent radar systems, has been well investigated. Accurate RTR at low signal-to-noise ratios (SNRs) still remains an open challenge. Most existing methods are based on a single radar or the homogeneous radar network, which do not fully exploit frequency-dimensional information. In this paper, a two-stream semantic feature fusion model, termed Multi-faceted Graph Attention Network (MF-GAT), is proposed to greatly improve the accuracy in the low SNR region of the heterogeneous radar network. By fusing the features extracted from the source domain and transform domain via a graph attention network model, the MF-GAT model distills higher-level semantic features before classification in a unified framework. Extensive experiments are presented to demonstrate that the proposed model can greatly improve the RTR performance at low SNRs.

==> prletters.tex <==
%%
%% This is file `prletters.sty',
%% generated with the docstrip utility.
%%
%% Copyright 2013 Elsevier Ltd
%%
%% This file is part of the 'Elsarticle Bundle'.
%% -------------------------------------------
%%
%% It may be distributed under the conditions of the LaTeX Project Public
%% License, either version 1.2 of this license or (at your option) any
%% later version.  The latest version of this license is in
%%    http://www.latex-project.org/lppl.txt
%% and version 1.2 or later is part of all distributions of LaTeX
%% version 1999/12/01 or later.
%%
%%
%% $Id: prletters.sty 66 2013-05-28 10:33:39Z rishi $
%%
\ProvidesPackage{prletters}
 \def\RCSfile{prletters}%
 \def\RCSversion{0.1}%
 \def\RCSdate{2013/05/13}%
 \def\@shortjnl{\relax}
 \def\@journal{Pattern Recognition Letters}
 \def\@company{Elsevier Ltd}
 \def\@issn{000-0000}
 \def\@shortjid{prletters}
\NeedsTeXFormat{LaTeX2e}[1995/12/01]

\@ifclassloaded{elsarticle}
{\typeout{elsarticle.cls is loaded...}}
{\errmessage{This package will work only with
  elsarticle.cls. So please load elsarticle.cls
  and try.}}

 \RequirePackage{geometry}
 \geometry{twoside,
  paperwidth=210mm,
  paperheight=280mm,
  textheight=693pt,
  textwidth=522pt,
  inner=15mm,
  top=15mm,
  headheight=50pt,
  headsep=10pt,
  footskip=12pt,
  footnotesep=28pt plus 2pt minus 6pt,
  columnsep=18pt
 }
 \global\let\bibfont=\footnotesize
 \global\bibsep=0pt
 \input{fleqn.clo}
\ifpreprint
\else
   \global\@twocolumntrue
\fi


\usepackage{multirow}
\usepackage{color}

\AtBeginDocument{
\def\elsarticletitlealign{flushleft}
}

%%
\def\snm#1{\textcolor{red}{#1}}

%% Title page header
\def\ps@PRlettersTitle{%
  \def\@oddhead{
\noindent\parbox[t]
  {\textwidth}{
  ~\hfill\thepage\\
  \rule{.8\textwidth}{.2pt}\\[.8ex]
   \includegraphics[scale=.8]{elsevier-logo}
   \hfill
    \raisebox{14pt}{\parbox{.5\textwidth}%
    {\centering {\large Pattern Recognition Letters}\\
    {\sf journal homepage: www.elsevier.com}}}
   \hfill
   \hspace*{.15\textwidth}\\[-4pt]
   \rule{\textwidth}{2pt}
}}
     \let\@evenhead\@empty
     \def\@oddfoot{}
     \let\@evenfoot\@oddfoot
}

\def\ps@headings{%
   \def\@oddhead{\mbox{~}\hfill\thepage}
   \let\@evenhead\@oddhead
   \let\@oddfoot\relax
   \let\@evenfoot\@oddfoot
}

% Header for other than title page.
\pagestyle{myheadings}

% History info
\let\@received\@empty
\let\@finalform\@empty
\let\@accepted\@empty
\let\@availableonline\@empty
\let\@communicated\@empty
\def\received#1{\gdef\@received{#1}}
\def\finalform#1{\gdef\@finalform{#1}}
\def\accepted#1{\gdef\@accepted{#1}}
\def\availableonline#1{\gdef\@availableonline{#1}}
\def\communicated#1{\gdef\@communicated{#1}}

\def\receivedhead{Received}
\def\acceptedhead{Accepted}
\def\finalformhead{Received in final form}
\def\availableonlinehead{Available online}
\def\communicatedhead{Communicated by}

% Article info
\def\articleinfobox{
    \parbox[t]{.25\textwidth}{%
    \vspace*{0pt}%
    \hrule%
    \vspace*{6pt}%
    \fontsize{8pt}{10pt}\selectfont%
    \textit{Article history}:\\
    \ifx\@received\@empty\relax
    \else
    \receivedhead~\@received\\
    \fi
    \ifx\@finalform\@empty\relax
    \else
    \finalformhead~\@finalform\\
    \fi
    \ifx\@accepted\@empty\relax
    \else
    \acceptedhead~\@accepted\\
    \fi
    \ifx\@availableonline\@empty\relax
    \else
    \availableonlinehead~\@availableonline
    \fi
    \ifx\@communicated\@empty\relax
    \\[-2pt]
    \else
    \par
    \vspace*{10pt}
    \communicatedhead~\@communicated
    \vspace*{12pt}
    \fi
    \hrule
    \vspace*{1pc}
    \unhbox\keybox}
}

% Preprint Maketitle
\long\def\pprintMaketitle{%
  \resetTitleCounters
  \def\baselinestretch{1}%
  \begin{\elsarticletitlealign}%
   \def\baselinestretch{1}%
    \vspace*{5pc}
    \Large\@title\par\vskip18pt
    \normalsize
  \ifdoubleblind
    \vspace*{2pc}
  \else
    \elsauthors\par\vskip10pt
    {\footnotesize\itshape\elsaddress}\par\vskip12pt
  \fi
\vspace*{-\baselineskip}%
\parbox[t]{\textwidth}{%
\parbox[t]{.25\textwidth}{\articleinfobox\\[3pt]\hrule}\hfill%
\parbox[t]{0.7\textwidth}{\rule{.6\textwidth}{.2pt}\vskip10pt
    \begin{tabular*}{.6\textwidth}{c@{}p{.9\textwidth}}
     \hspace*{7pt}&ABSTRACT\\[8pt]
    \hline\\[-8pt]
    \end{tabular*}
    \hspace*{13.5pt}\parbox[t]{.577\textwidth}{\unhbox\absbox}
    \\[3pt]\rule{.7\textwidth}{.2pt}%\vskip10pt%
    }}%
  \end{\elsarticletitlealign}%
%\rule{.6\textwidth}{.2pt}%\vskip10pt%
  \vspace*{2pc}
    \printFirstPageNotes
}


% Maketitle
\long\def\MaketitleBox{%
  \resetTitleCounters
  \def\baselinestretch{1}%
  \begin{\elsarticletitlealign}%
   \def\baselinestretch{1}%
    \vspace*{7.5pc}
    \Large\@title\par\vskip18pt
    \normalsize
  \ifdoubleblind
    \vspace*{2pc}
  \else
    \elsauthors\par\vskip10pt
    {\footnotesize\itshape\elsaddress}\par\vskip12pt
  \fi
\vspace*{-\baselineskip}%
\parbox[t]{\textwidth}{%
\parbox[t]{.25\textwidth}{\articleinfobox\\[3pt]\hrule}\hfill%
\parbox[t]{0.7\textwidth}{\rule{.7\textwidth}{.2pt}\vskip10pt
    \begin{tabular*}{.7\textwidth}{c@{}p{.7\textwidth}}
     \hspace*{7pt}&ABSTRACT\\[8pt]
    \hline\\[-8pt]
    \end{tabular*}
    \hspace*{13.5pt}\parbox[t]{.677\textwidth}{\unhbox\absbox}%
    \\[3pt]\rule{.7\textwidth}{.2pt}%\vskip10pt%
    }}
  \end{\elsarticletitlealign}%
  \vspace*{2pc}
    \printFirstPageNotes
}

\long\def\finalMaketitle{%
  \resetTitleCounters
  \def\baselinestretch{1}%
   \MaketitleBox
   \thispagestyle{PRlettersTitle}%
  \gdef\thefootnote{\arabic{footnote}}%
  }


\def\printFirstPageNotes{%
  \def\snm##1{##1}%
  \iflongmktitle
   \let\columnwidth=\textwidth\fi
  \ifdoubleblind
  \else
  \ifx\@tnotes\@empty\else\@tnotes\fi
  \ifx\@nonumnotes\@empty\else\@nonumnotes\fi
  \ifx\@cornotes\@empty\else\@cornotes\fi
  \ifx\@elseads\@empty\relax\else
   \let\thefootnote\relax
   \footnotetext{\ifnum\theead=1\relax
      \textit{e-mail:\space}\else
      \textit{e-mail:\space}\fi
     \@elseads}\fi
  \ifx\@elsuads\@empty\relax\else
   \let\thefootnote\relax
   \footnotetext{\textit{URL:\space}%
     \@elsuads}\fi
 \fi
  \ifx\@fnotes\@empty\else\@fnotes\fi
  \iflongmktitle\if@twocolumn
   \let\columnwidth=\Columnwidth\fi\fi
}

% Abstract
\renewenvironment{abstract}{%
  \global\setbox\absbox=\hbox\bgroup%
  \hsize=.4\textwidth%
  \hskip-1pt}
 {\newline
   \mbox{~}\hfill\copyright~\the\year\
   Elsevier~Ltd.~All~rights~reserved.\egroup%
 }



% Keyword
\def\keyword{%
  %\def\sep{\newline}%
  \def\sep{\unskip\ignorespaces,\space}%
  \def\MSC{\@ifnextchar[{\@MSC}{\@MSC[2000]}}%
%  \def\@MSC[##1]{\leavevmode\hbox {\it ##1~MSC:}\newline}%
  \def\@MSC[##1]{\leavevmode\hbox {\it ##1~MSC:}~}%
  \def\JEL{\newline\leavevmode\hbox {\it JEL:\space}}%
  \def\KWD{%
   \vspace*{10pt}\newline
%   \leavevmode\hbox {\it Keywords:}\newline}%
   {\it Keywords:}~}%
  \global\setbox\keybox=\hbox\bgroup\hsize=.3\textwidth%
  \fontsize{8pt}{10pt}\selectfont%
  \parskip\z@%
  \noindent%
  \ignorespaces}
\def\endkeyword{\egroup}

%% Other customization

% Enumerate
\def\labelenumii{\labelenumi.\arabic{enumii}}

% Caption
\def\figurename{Fig.}

\long\def\@makecaption#1#2{%
  \vskip\abovecaptionskip\footnotesize\bfseries
  \sbox\@tempboxa{#1.~#2}%
  \ifdim \wd\@tempboxa >\hsize
    #1.~#2\par
  \else
    \global \@minipagefalse
    \hb@xt@\hsize{\hfil\box\@tempboxa\hfil}%
  \fi
  \vskip\belowcaptionskip}

\AtBeginDocument{\ifpreprint
 \advance\baselineskip by 12pt
\fi}

\def\TM{$^{\rm TM}$}

